MoDA: Map style transfer for self-supervised Domain Adaptation of embodied agents

We propose a domain adaptation method, MoDA, which adapts a pretrained embodied agent to a new, noisy environment without ground-truth supervision. Map-based memory provides important contextual information for visual navigation, and exhibits unique spatial structure mainly composed of flat walls and rectangular obstacles. Our adaptation approach encourages the inherent regularities on the estimated maps to guide the agent to overcome the prevalent domain discrepancy in a novel environment. Specifically, we propose an efficient learning curriculum to handle the visual and dynamics corruptions in an online manner, self-supervised with pseudo clean maps generated by style transfer networks. Because the map-based representation provides spatial knowledge for the agent's policy, our formulation can deploy the pretrained policy networks from simulators in a new setting. We evaluate MoDA in various practical scenarios and show that our proposed method quickly enhances the agent's performance in downstream tasks including localization, mapping, exploration, and point-goal navigation.

==> 3_method.tex <==
\section{Method}



\begin{figure}[t]
\centering
\includegraphics[width=1.\columnwidth]{Figures/temp_fig1.png}
\caption{ Overview}
\label{fig:overview}
\end{figure}

Given a pretrained agent from a noiseless simulator, MoDA transfers the agent to unseen, noisy environments for robust visual navigation. 
We propose a self-supervised, online domain adaptation method which learns from map style transfer.
MoDA is designed to learn the visual corruptions, changes on RGB inputs, from the egocentric maps and the dynamics corruptions, uncertainty on pose estimation, from the global maps where the two corruptions are learned in a curriculum. 
In this section, we describe our navigation agent, the various types of corruptions, our map style transfer networks and, lastly, the learning curriculum of our domain adaptation method.   

\subsection{Visual Navigation with Spatial Map Memory}
% egomapper, globalmapper? 
% egomapper, pose estimator? 
%in the figure, indicate the added part of self-supervised learning with line color (noises + self supervision) 
MoDA proposes an integrated domain adaptation approach for visual and dynamic corruptions, which formulates self-supervision on occupancy grid maps. 
Our approach can be easily applied to many map-based navigation agents.
As shown in Fig.~\ref{fig:overview}, the hierarchical architecture of map-based agents generates egocentric maps and global maps which we utilize to learn for the visual and dynamic corruptions accordingly. 
At each step, the RGB observation $o_t$ is given as an input to the mapping model which predicts the egocentric map $m_t$. 
We define our mapping model $f_{\mathbbm{m}}$ as 
\begin{align}
    f_{\mathbbm{m}}(o_{t}) = m_{t}.
\end{align}
Given the odometry sensor measurement $s_t$, the localization model predicts the 2D pose, $p_t=(x,y,\phi)$, where
$(x,y)$ indicates the 2D coordinate and $\phi$ denotes the 1D orientation.
Note that the predicted egocentric maps from the previous step and the current step are given to help the pose prediction. 
The localization model $f_{\mathbbm{l}}$ is represented as 
\begin{align}
    f_{\mathbbm{l}}(s_{t}, m_{t-1}, m_{t}) =  \hat{p}_{t},
\end{align}
where $\hat{p}_{t}$ indicates the predicted pose. 
Finally, the predicted egocentric maps from the mapping model transformed by the estimated poses from the localization model are combined at each step to generate a new global map. Thus, the global mapper $T$ is defined as 
\begin{align}
    T(m_{t}, \hat{p}_{t}, M_{t-1}) = M_{t}.
\end{align}
Then the policy module $\pi_\psi$ plans an action $a_t \in \mathcal{A}$ from the allocentric understanding derived from the global map $M_{t}$ and the agent's current pose $\hat{p}_t$. 
\begin{align}
    \pi_{\psi}(M_{t},\hat{p}_{t}) = a_{t}.
\end{align}
Our agent plans a discrete action from a set, $\mathcal{A}$=\{Forward, Turn Right, Turn Left\}.

The agent trains the mapping, localization and policy module in an ideal environment with the ground truth information of egocentric maps and poses.
However, in the realistic environments, the overall architecture is disturbed by two main types of corruptions. 
The visual corruptions on RGB observations make it difficult to predict egocentric maps and the dynamic corruptions on odometry readings and actuation degrades the pose estimation. 
As the modular pipeline decouples the policy from the perturbations in measurements, our proposed domain adaptation method, MoDA, only fine-tunes the mapping and localization models which are tightly coupled to the corruptions. 
Moreover, the hierarchical order of mapping and localization models allows us to design the efficient learning curriculum which adapts to the visual and dynamic domain changes in a sequential order. 


\subsection{Visual and Dynamic Corruptions}
\label{sec:corruptions}
 %mp3d, low-lighting = corruptions? 
Visual corruptions on RGB observations disturb the embodied agent's egocentric perception.
We carefully select three types of realistic corruptions to properly represent the wide varieties of possible visual variations in the real world [robustnav].
The agent is pretrained in a noiseless Gibson scenes. 
First, we evaluate if our agent can adapts to image quality degradation. 
It is a realistic visual corruption which may be caused by the mounted camera's conditions.
We add speckle noise, modeled as additive noise, to generate a low-quality RGB observations. 
The second type of perturbations is low-lighting condition. 
Lighting of a scene is the most common source of visual variations. 
%In simulators, the 3D scans come with lighting baked into the texture where the agent is only allowed to train in the original lighting condition.
We show if our agent can be transferred to low-lighting scenes by adjusting the contrast and brightness of the input RGB image. 
Lastly, we evalute if our pretrained agent from Gibson scenes can generalize to large-scale scenes from Matterport3D. 
While the Gibson scenes consists of scans collected from offices, the scenes in Matterport3D generally consists of large-scale homes. % different cameras used
In figure~\ref{fig:visualcorruptions}, the RGB observations obtained from the three visual changes, namely, \textit{low-quality}, \textit{low-lighting} and \textit{large-scale}, are visualized.  

\begin{figure}[t]
\centering
\includegraphics[height=3.5cm]{Figures/temp_fig5.png}
\caption{ Visual Corruptions: low-quality, low-lighting, large-scale}
\label{fig:visualcorruptions}
\end{figure}

Dynamic corruptions degrade the agent's pose estimation accuracy. 
The actuation and odometry sensor noises are two main dynamic corruptions expected in all realistic settings. 
Here, we describe the two noises and how they disturb the agent's performance. 
First, the actuation noise interrupts an agent from reaching the target location. 
The agent is no longer able to deduce the agent's ground-truth location simply from the given control commands. 
After an action, the agent's ground-truth pose is defined as 
\begin{align}
    (x_{t+1},y_{t+1},\phi_{t+1}) = (x_{t}, y_{t}, \phi_{t}) + (u_x,u_y,u_\phi) + \epsilon_{act},
    \label{eq:pose_actuation_noise}
\end{align}
where the $(u_x,u_y,u_\phi)$ and $\epsilon_{act}$ indicate the intended action control and actuation noise.  
Additionally, the odometry sensor noise $\epsilon_{sen}$ disturbs the agent from accurately perceiving its own movement. 
The final pose reading with the odometry sensor noise $\epsilon_{sen}$ is erroneously measured as 
\begin{align}
   (x_{t+1}',y_{t+1}',\phi_{t+1}') = (x_{t+1},y_{t+1},\phi_{t+1}) + \epsilon_{sen}. 
   \label{eq:pose_odometry_noise}
\end{align} 
Many studies have presented the modeling work of realistic dynamic corruptions. 
In our work, we employ the noise parameters modeled from actual physical deployment[] and draw each noise form a Gaussian Mixture Model. 



\subsection{Unpaired map-to-map translation Network}
The main objective of our self-supervised domain adaptation is to translate maps from the new, noisy domain to the noiseless domain in the absence of paired data as shown in Fig ~\ref{fig:style-transfer}.
As our maps are simply represented as gray-scale images, we adopt the unpaired image-to-image translation network suggested in [CycleGAN] to train map-to-map translation networks. 
A pretrained agent can store a collection of ground-truth maps $D_{gt}$ from noiseless simulator. 
When deployed in a new environment, the agent collects another set of map data $D_{noisy}$ which is generated amidst visual and dynamic corruptions. 
Given the two sets of map dataset, We train the networks to capture the structural regularities of indoor scenes from the collection of ground-truth maps and translate the learned characteristics into the collection of noisy maps. 
Reasoning about the stylistic difference between two collections, rather than learning to translate from one map to the other, allows us to formulate the domain adaptation method in a complete self-supervised manner. 
% Moreover, our maps in the form of gray-scale images allow the networks to easily learn the style stably in a short amount time.   

More specifically, we learn two map-to-map translation networks. 
First, the style-transfer network for egocentric maps $S_{ego}$ is trained to transfer the style of ground-truth egocentric maps into the egocentric maps generated in visually noisy environments.
The magnified view of the environment helps the agent to learn the visual detailed structure of the indoor scene. 
% detailed style learned from egocentric view? 
For the egocentric maps, we learn to the network over the total explored area. 
We empirically find that it is difficult to train the network over the obstacle-aware ego maps as the map images consist only about 6\% of nonzero values on average. 
The global map style-transfer network $S_{global}$ is trained to learn the stylistic characteristic from the set of ground-truth global maps and translate the newly predicted global maps from the noisy environments.
The style-transferred map constrains the agent from making noisy structured map and back-propagates the self-supervised loss to restrict the pose estimator from making erroneous predictions. 

% structural regularities learned from long-horizon navigation? 
% helps the agent to learn the pose estimation over the maps generated from temporally different steps


\begin{figure}[t]
\centering
\includegraphics[height=4.0cm]{Figures/temp_fig3.png}
\caption{ Style transfer network overview}
\label{fig:style-transfer}
\end{figure}


\subsection{Curriculum Learning for Domain Adaptation} 

\paragraph{Curriculum Learning}
MoDA adapts the pretrained agent in a curriculum following the hierarchical structure of map-based models which concatenate the predicted egocentric maps to generate a global map. 
Egocentric maps are predicted solely from the agent's visual perception. For visual domain adaptation, we adapt the feature extractor of mapping model $f_{\mathbbm{m}}$ using the style-transfer loss formulated on the egocentric maps along with the loss encouraging the flip consistency on the RGB observation. 
In the next step, the agent fine-tunes the localization model $f_{\mathbbm{l}}$ for dynamic domain adaptation. 
We formulate loss on the global maps which learn from the global style-transfer network and the temporal consistency over the agent's trajectories. 
As shown in figure ~\ref{fig:curriculum_learning}, our self-supervised adaptation method fine-tunes for the new visual and dynamic domain sequentially during its initial stage of deployment. 
The transferred agent then stably perform various navigation tasks in the new, noisy environment.  

\paragraph{Visual Domain Adaptation}
According to the learning curriculum, we first adapt the mapping model for unknown visual changes in the new environments. 
At each step, the predicted egocentric map $m_{t}$ is given as an input to the egocentric map style-transfer network $S_{ego}$, which generates a style transferred map. 
During the visual domain adaptation stage, the estimated map is then compared to the transferred map and formulates the ego style transfer loss $L_{ego,st}$.
With $T_{v}$ indicating the visual domain adaptation time, the ego style transfer loss is defined as 
\begin{align}
   \mathcal{L}_{ego,st} & = \sum_{t=0}^{T_{v}} \| m_{t} - S_{ego}(m_{t}) \|_{2}.  
\end{align}
In addition, we learn the feature extractor $F$ of the mapping model along with a consistency loss to stabilize the training. 
The flip consistency loss $L_{fc}$ assumes that the feature extractor should make consistent predictions over the flipped observations. Specifically, when a horizontally flipped RGB observation, $I_{flip,t}$, and a non-flipped original observation, $I_{t}$, are given as inputs, the estimated egocentric maps should be equal but flipped.
We, therefore, define our flip consistency loss as 
\begin{align}
   \mathcal{L}_{fc} & = \sum_{t=0}^{T_{v}} \| F(I_{t}) - flip ( F ( I_{flip,t} )) \|_{2}, 
\end{align}. 
Therefore, the mapping model of the pretrained agent is transferred to the visual corruptions with the visual domain loss, $L_{VD}$.
The overall objective of visual domain adaptation is
\begin{align}
    \mathcal{L}_{VDA} &= \lambda_{ego,st} \mathcal{L}_{ego,st} + \lambda_{fc} \mathcal{L}_{fc}.
\end{align}
The exact values for hyper-parameters are provided in the supplementary material.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figures/temp_fig2.png}
\caption{Curriculum learning}
\label{fig:curriculum_learning}
\end{figure}

\paragraph{Dynamic Domain Adaptation}
In the next stage, we adapt the agent's pose estimator to the dynamic corruptions that are present in the new environment.
The agent generates a global map over its trajectory and encodes the predicted pose information onto the map. 
Thus, learning the structural loss from the style transfer network, the agent can inversely learn to estimate more accurate pose. 
Given the estimated and style-transferred global maps, the global style transfer loss, $L_{global,st}$ is formulated as
\begin{align}
  \mathcal{L}_{global,st} & = \sum_{t=T_{v}+1}^{T_{d}} \| M_{t} - S_{global}(M_{t}) \|_{2}.  
\end{align}
where $T_{d}$ denotes the ending time of dynamic domain adaptation.
Moreover, we encourage the agent to generate consistent global maps over time. 
As the pose error accumulates over time, the global map generated in the earlier step encodes more accurate pose information over the global map generated in the later step. 
The temporal consistency loss $L_{tc}$ compares the generated global map to the map from the previous time-step, and it is defined as
\begin{align}
   \mathcal{L}_{tc} & = \sum_{t=T_{v}+1}^{T_{d}} \| M_{t} - M_{t-1} \|_{2}.
\end{align}
Therefore, the full objective of dynamic domain adaptation becomes 
\begin{align}
    \mathcal{L_{DDA}} &= \lambda_{global,st} \mathcal{L}_{global,st} + \lambda_{tc} \mathcal{L}_{tc}.
\end{align}
%MSE for all suggested loss.


==> 4_experiments.tex <==
\section{Experiments}
We evaluate the proposed method in three scenarios where, in all cases, the pretrained agent needs to transfer to the new environment with both visual and dynamic corruptions. 
In all scenarios, the dynamic corruptions consist of both odometry sensor and acutation noises, as the two noises are expected in all realistic environments. 
For dynamic corruptions, we use the model generated from real deployment of LoCoBot~\cite{} in the the previous work ~\cite{chaplot2020learning,kadian2020sim2real}. 
Each environment is distinguished by its visual domain.
The three visual domains explained in Section~\ref{sec:corruptions}, low-quality, low-lighting, and large-scale visual variations are observed in each new environment. 
We show the validity of our domain adaptation method using the visual navigation agent proposed in Active Neural SLAM~\cite{chaplot2020learning} as it is widely-used in many studies[]. 
However, MoDA is applicable to various visual navigation agents with map-like memory. 

\paragraph{Experiment Setup} 
We use Habitat simulator[] with the scenes from Gibson[] and Matterport3D dataset[].
The pretrained agent is trained on the standard train split[] of Gibson dataset with the ground-truth supervision. 
For our experiments, we split the unseen scenes of Gibson and Matterport3D for adaptation and evaluation. 
We implement the self-supervised learning method on the navigation model[ANS] using Pytorch[] to allow fine-tuning from the suggested map style transfer loss and consistency loss. 
The adaptation, which completes within x minutes, is accelerated with an RTX 2080 GPU. 
The list of scenes used for each split and additional details of experiments are provided in the supplementary material.

We evaluate MoDA with various metrics. 
We report the transferred agent's localization and mapping performance in the new, noisy environment.  
Following ~\cite{campbell2018globally,campbell2019alignment}, the localization measures the median difference of translation ($x,y$) and rotation ($\phi$) for each episode.
The mapping performance is evaluted with the mean squared error (MSE) of the generated occupancy grid maps compared to the ground-truth maps.  
MoDA is an online domain adaptation method applied during the initial stage of deployment. 
However, as the trajectory generated by the agent varies by its navigation performance, we cannot make a fair comparison of localization and mapping in an online manner. 
Thus, we store trajectories of a  pretrained agent in a noisy environment and evaluate each agent's localization and mapping performance on the stored trajectories.
Moreover, the downstream navigation task performance is evaluated to show that the enhancement in localization and mapping also leads to the improvement in the policy model. 
Following the task setup proposed by [], we report the exploration performance, the area coverage and area ratio explored within a fixed number of steps. 
We also add a metric which reports the collision ratio over the agent's exploration steps. 
Mainly, embodied agents navigation performance is widely evaluated using PointNav task as suggested in [].  
In PointNav, the agent performs a fundamental navigation task. A target location relative to the agent's starting point is given and it navigates to reach the target within the designated number of steps. 
Here, the ratio of successful episodes and Success weighted by Path Length(SPL)[] are reported. 
In all our experiments, our agents perform a task for 1000 steps. 

\paragraph{Baselines}
We extensively compare our domain adaptation method with various baselines.
We deploy the pre-trained model in a new, noisy environment with visual and dynamic corruptions. 
Without any adaptation, "No adaptation(\textbf{NA})" reflects the performance degradation of the pretrained model due to the domain gap. 
NA serves as the lower bound of our proposed model's performance. 
"GT Train (\textbf{GT})" model is fine-tuned with ground-truth supervised setting in the new environment. 
Even though the ground-truth labels are not available in the realistic scenario, we train the model to provide the performance upper bound.
Next, the "Domain Randomization(\textbf{DR})" model fine-tunes our pre-trained model in a randomized domain. The various combinations of a visual corruption and a dynamic corruption are randomly exposed to the pre-trained model with ground-truth supervision.
The DR model requires the modeling of multiple visual and dynamic noises.

We also compare our method against two other baselines which fine-tune the agent without ground-truth supervision. 
[PAD] suggests a domain adaptation method which trains the agent with an auxiliary task during the pre-training stage and during the deployment. 
As suggested, we implement a separate rotation prediction task which rotates the input RGB observation by the angle randomly selected from {0,90,180,270} and makes the prediction of rotation angle. 
With the ground-truth rotation angle provided, the auxiliary task can be continuously trained during deployment to fine-tune the feature extractor. 
However, we empirically observed that this adaptation method which we refer to as "Policy Adaptation during Deployment(\textbf{PAD})" degrades the pre-trained model's performance. 
Thus, we jointly adapt the model's auxiliary task and the pose estimator with our dynamic adaptation process.
Lastly, Lee et al.[] suggests a self-supervised domain adaptation method which formulates the global map consistency loss to learn dynamic corruptions. 
It provides an offline adaptation method which works on stored trajectories. 
This "Global Map Consistency(\textbf{GMC})" provides a comparable map-based adaptation model for our model. %Offline
However, GMC requires the agent to navigate in round-trip trajectories and inefficiently allows the adaptation only during its backward path. 
%GMC model also does not provide any solution to adapt to visual corruptions.
\input{Tables/table_1} 

\paragraph{Generalization and Specialization}
We investigate MoDA in two experimental settings similarly following the setup proposed in [SEAL].
In our main experiment, \textit{generalization} adapts the agent in a set of unseen, noisy scenes. 
We call it our adaptation split. 
It is then evaluated in different set of unseen scenes, the test split, but with the same visual and dynamic corruptions. 
In addition, we evaluate if the agent can be transferred to the same scenes from the adaptation split. 
In \textit{specialization}, the trained models are evaluated in the same scenes from adaptation split but on different episodes which start the agent from a different initial position. 

\subsection{Task Adaptation to Noisy Environments: Generalization}
We transfer the pretrained agent to the adaptation split which consists of new scenes with unknown visual and dynamic corruptions. 
The agent's performance is then evaluated in a different set of new scenes but with the same environmental corruptions. 
%redundant? 
This generalization setting tests whether the adaptation method properly transfers the agent to the existing visual and dynamic corruptions, rather than over-fitting the agents to the given scenes.
We compare our agent adapted with MoDA against all baselines, in all three scenarios suggested.

In Table 1, we show that our agent referred as "MoDA" outperforms the NA model in all scenarios and in all evaluation metrics. 
The improvement in egocentric map prediction and pose estimation leads to the enhanced result in global map generation and in the downstream navigation tasks.
The DR model, while showing the least improvement in localization, outperforms the other self-supervised baselines, GMC and PAD, in exploration ratio. 
[on evaluation~] studies how the collision setting in habitat which allows the agent's sliding causes the performance gap of the agent in simulators and reality.
We believe that the sliding effect after each collision lead to the inconsistent exploration performance and additionally report the collision ratio over the total steps. 
As expected, DR model results in the highest collision ratio which supports the conclusion that our MoDA model, outperforming in both of the original exploration metrics and in collision ratio properly adapted to the new environment. 
PAD model underperforms compared to NA model in mapping and final navigation tasks.  
However, we observe that PAD, jointly trained for dynamic corruptions with our proposed method, results in outstanding localization performance. 
The result shows that our dynamic adaptation method can be easily combined with other visual domain adaptation method.   
Lastly, GMC model shows the most comparable improvement against our MoDA model. 
While GMC mandates impractical round-trip trajectories, the evaluation of GMC shows the efficiency of the dynamic domain adaptation approach which formulates self-supervision loss on maps. 

In figure [], we show the visualization of the estimated pose trajectory and reconstructed global maps generated by the agents observing the same sequence of RGB observations and odometry sensor readings.
The qualitative result is reported for the scenario where the new environment consists of low-quality image and dynamic corruptions. 
Our model better aligns with the ground-truth, confirming its outstanding performance compared to the baselines. 
Our online, self-supervised adaptation method compensates for both visual and dynamic corruptions, resulting in performance enhancement almost comparable to GT baseline which is not trainable in a realistic environment with no ground-truth data. 

\input{Tables/table_1_spec} 
\input{Tables/table_2}

\subsection{Task Adaptation to Noisy Environments: Specialization}
In specialization, the models are evaluated on the same scenes in the adaptation split. 
However, the agents start navigating from a different initial location. 
This specialization setting represent the real-world deployment in which an embodied agent may be deployed and continuously used in the same scenes. 
In Table 2, we report the transferred agent's performance in localization, mapping and PointNav task in all three experiment scenarios.
Interestingly, in contrast to the generalization result, PAD shows improvement in PointNav metric for low-light and large-scale environment. 
We can deduce that the visual adaptation method used in PAD is more effective in learning the scene but not the added visual corruptions.  
Still, our agent, compared to the baselines, exhibits an outstanding performance improvement, almost comparable to the GT model.
Therefore, fine-tuning the agent during a short amount of time (time), MoDA provides a powerful, integrated adaption method for closing the domain gap from visual and dynamic corruptions available in realistic environment. 

\subsection{Ablation study}
In this section, we ablate each loss formulated for visual and dynamic corruptions.
The result in Table 2 is evaluated in low-image quality scenario. 
The overall experiment setup is the same as generalization. 
Staring from the pretrained agent, we add each loss used and evalute the performance in localization, mapping and PointNav. 
The pretrained agent only trained for flip consistency loss shows the performance improvement in localization and the final PointNav task.
The addition of ego style-transfer loss then enhances the performance in all metrics. 
Note that this ablated model with flip consistency and ego style-transfer loss exhibits the performance of the agent only adapted for visual domain corruptions. 
The adaptation for visual perturbations, which targets at predicting more accurate egocentric maps, also leads to the improvement in the subsequent evaluation tasks, localization, global map prediction and PointNav performance. 
The visually adapted agent is then trained with the temporal consistency loss. 
The temporal consistency loss itself is able to enhance the agent's performance but the global style transfer stably enhances the agent's overall performance in all metrics. 

\begin{figure}[t]
\centering
\includegraphics[height=15.0cm]{Figures/figure5.png}
\caption{ Qualitative result of mapping and localization}
\label{fig:qual_result}
\end{figure}


% synergy 
% style adjusted global map  -> capture the temporal difference more clearly

